Scalable Tucker Factorization for Sparse Tensors - Algorithms and Discoveries

Given sparse multi-dimensional data (e.g., (user, movie, time; rating) for movie recommendations), how can we discover latent concepts/relations and predict missing values? Tucker factorization has been widely used to solve such problems with multi-dimensional data, which are modeled as tensors. However, most Tucker factorization algorithms regard and estimate missing entries as zeros, which triggers a highly inaccurate decomposition. Moreover, few methods focusing on an accuracy exhibit limited scalability since they require huge memory and heavy computational costs while updating factor matrices. In this paper, we propose P-Tucker, a scalable Tucker factorization method for sparse tensors. P-Tucker performs alternating least squares with a row-wise update rule in a fully parallel way, which significantly reduces memory requirements for updating factor matrices. Furthermore, we offer two variants of P-Tucker: a caching algorithm P-Tucker-Cache and an approximation algorithm P-Tucker-Approx, both of which accelerate the update process. Experimental results show that P-Tucker exhibits 1.7-14.1x speed-up and 1.4-4.8x less error compared to the state-of-the-art. In addition, P-Tucker scales near linearly with the number of observable entries in a tensor and number of threads. Thanks to P-Tucker, we successfully discover hidden concepts and relations in a large-scale real-world tensor, while existing methods cannot reveal latent features due to their limited scalability or low accuracy.

==> dfn.tex <==
%\usepackage{ntheorem}


\newtheorem{observation}{Observation}
%\newtheorem{conjecture}{Conjecture}
\newtheorem{problem}{Problem}
\newtheorem{algo}{Algorithm}
%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}

\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\SetKwInOut{Map}{Map}
\SetKwInOut{Reduce}{Reduce}
\SetKwInOut{Partition}{Partition}

%\newtheorem{proof}{Proof}
\newtheorem{defi}{Definition}
\newcommand{\T}[1]{\boldsymbol{\mathscr{#1}}}   %% Tensor macro
\newcommand{\mb}[1]{\boldsymbol{\mathscr{#1}}}

\newcommand{\method}{\textsc{P-Tucker}\xspace}
\newcommand{\hide}[1]{}
%\newcommand{\comment}[1]{{\tiny #1 }}
\newcommand{\semihide}[1]{{\tiny #1}}
%\newcommand{\reminder}[1]{{\em *** #1 ***}}
\newcommand{\reminder}[1]{{\textsf{\textcolor{red}{[#1]}}}}
\newcommand{\ukang}[1]{{\textsf{\textcolor{red}{[From U: #1]}}}}

\newcommand{\krp}[2]{ \left( \mathbf{#1}\odot\mathbf{#2} \right)}

\def\blambda{\mbox{\boldmath ${\lambda}$}}
\newcommand{\makeclean}{
    \renewcommand{\reminder}[1]{}
}

%\newcommand{\QED}{ \hfill {\bf QED}}
\newcommand{\tight}{ \setlength{\itemsep}{-1.0\itemsep} }
    % makes lists tighter

\newcommand{\tsection}[1]{ \vspace{-1.0\baselineskip} \section{#1} \vspace{-2mm} }
\newcommand{\tsubsection}[1]{ \vspace{-0.75\baselineskip} \subsection{#1} \vspace{-0.5\baselineskip} }

\newcommand{\tensor}[1]{\boldsymbol{\mathscr{#1}}}   %% Tensor macro
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\vect}[1]{\mathbf{#1}}

\newcommand{\argmin}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{min}}\;}
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{max}}\;}

% naming conventions
\newcommand{\hadi}{{\cal HADI}\xspace}
\newcommand{\mapreduce}{\textsc{MapReduce}\xspace}
\newcommand{\hadoop}{\textsc{Hadoop}\xspace}

\newcommand{\PassA}{{\tt Stage1}\xspace}
\newcommand{\PassAMap}{{\tt Stage1-Map}\xspace}
\newcommand{\PassARed}{{\tt Stage1-Reduce}\xspace}
\newcommand{\PassB}{{\tt Stage2}\xspace}
\newcommand{\PassBMap}{{\tt Stage2-Map}\xspace}
\newcommand{\PassBRed}{{\tt Stage2-Reduce}\xspace}
\newcommand{\PassC}{{\tt Stage3}\xspace}
\newcommand{\PassCMap}{{\tt Stage3-Map}\xspace}
\newcommand{\PassCRed}{{\tt Stage3-Reduce}\xspace}

\newcommand{\diameter}{{\tt diameter}}
\newcommand{\npairs}{{\tt npairs}}
\newcommand{\gcc}{{\tt gcc}}
\newcommand{\entropy}{{\tt entropy}}
% \newcommand{\nedges}{{\tt nedges}}
\newcommand{\sv}{{\mbox{$\lambda_1$}}}
\newcommand{\avgd}{{\tt avgd}}

% math symbol definitions
\newcommand{\nnodes}{N}     % number of nodes
\newcommand{\nedges}{E}     % number of edges
\newcommand{\deff}{{d_{eff}}}   % effective diameter
\newcommand{\Er}{{E_{r}}}   % number of retained edges
\newcommand{\Nr}{{N_{r}}}   % number of retained nodes
\newcommand{\Nc}{{N_c}}   % number of nodes at critical point
\newcommand{\Ec}{{E_c}}   % number of nodes at critical point
\newcommand{\Ngcc}{{N_{gcc}}} % number of nodes in gcc, at critical poing
\newcommand{\NPairc}{{N_{NPAIRS}}} % number of reachable pairs, at critical poing
\newcommand{\dc}{{d_{c}}} % diameter at critical point
\newcommand{\Lambdac}{{\lambda_{c}}} % First eigenvalue at critical point
% \newcommand{\RED}{ {\em RED } } % random edge deletion
% \newcommand{\FED}{ {\em FED } } % friendly edge deletion
% \newcommand{\HED}{ {\em HED } } % hostile edge deletion


\newcommand{\ben}{\begin{enumerate*}}
\newcommand{\een}{\end{enumerate*}}
\newcommand{\bit}{\begin{itemize*}}
\newcommand{\eit}{\end{itemize*}}

% shorthands
\newcommand{\citationsds}{{CITATIONS}}
\newcommand{\epinionsds}{{EPINIONS}}
\newcommand{\patentsds}{{PATENTS}}
\newcommand{\net}[1]{{\textsc{#1}}}

%\newcommand{\QED}{\hfill $\Box$ \hfill}
\newcommand{\model}{\textsc{CommunityConnection}}

% modified
\newcommand{\modi}[1]{\textcolor{red}{#1}}
